Multilevel Stochastic Plug-and-Play for Sparse-View CT Reconstruction

Sparse-view computed tomography (SVCT) reduces radiation exposure and acquisition time, but the limited number of projection views makes the reconstruction problem severely ill-posed and leads to streak artifacts when analytical methods are used. Plug-and-Play (PnP) methods combine data fidelity with learned image priors, while stochastic PnP methods use re-noising to reduce the mismatch between denoiser training inputs and reconstruction iterates. However, these methods often require many iterations, which limits their practical efficiency. In this work, we propose multilevel (ML) Stochastic Plug-and-Play (ML-SPnP), a ML stochastic PnP method for SVCT reconstruction formulated on wavelet multiresolution analysis (MRA) approximation spaces. The method combines coarse-to-fine initialization with a finite sequence of ML corrections using resolution-specific denoisers. Under suitable assumptions, the fine-level iterations following the finite ML phase inherit the convergence guarantees of the underlying stochastic PnP algorithm. Experiments on two CT datasets with 20-50 projection views show that ML-SPnP achieves reconstruction quality comparable to the evaluated stochastic PnP methods, while generally requiring less reconstruction time. These results support ML acceleration as an effective strategy for reducing the computational cost of stochastic PnP reconstruction. The code will be made publicly available at https://github.com/antoinedepaepe/ml-spnp.

==> content/proof_convergence.tex <==
In the following we assume that the measurement data $\boldy$ is fixed, such that all expectation are taken conditionally to $\boldy$. To simplify,the notations, we opted for not explicitly writing the conditioning in $\boldy$. 

We analyse the asymptotic properties of ML-SPnP. For this purpose, we consider the case with an iteration dependent step size $\delta_k$, $k\ge K_{\mathrm{ML}}$, that is to say, only after the \gls{ML} steps, for the fine-level update. We also consider the setting of \citeauthor{renaud2025convergence}~\cite{renaud2025convergence},
\begin{displaymath}
	\sum_k \delta_k = + \infty \, , \quad \sum_k (\delta_k)^2 = 0 \, ,
\end{displaymath}
that is to say, $\delta_k \to 0$ but not too rapidly, and we consider $h = h_{\sigma,0}$ \eqref{eq:obj_l}. While \citeauthor{renaud2025convergence} do not demonstrate the convergence of $\boldx^{(k)}$ defined Algorithm~\ref{algo:wml_spnp} to a minimizer for $h$, it is possible to demonstrate  that there exists a subsequence for which the gradient of the objective tends to zero almost surely. 
\begin{proposition}
	We assume that $\mathbb{E} \left[ h\left( \boldx^{( K_{\mathrm{ML}})} \right)\right] < +\infty$. Under suitable smoothness assumptions (Lipschitz continuity for $D_{\sigma,\ell}$), for $f=f_0,f_1,\dots,f_L$ defined in \eqref{eq:obj_l}, and $\delta^{K_{\mathrm{ML}}}$ small enough, the sequence of estimates at fine level $(\boldx_0^{(k)})_k$ from Algorithm~\ref{algo:wml_spnp} verifies 
	\begin{equation}\label{eq:step}
		\liminf_{k\to\infty}  \left\| \nabla h \left(\boldx_0^{(k)} \right)  \right\|_2 = 0 \,  \quad \text{almost surely given $\boldy$}.
	\end{equation}
	% and iteration-dependent step $\delta^k$.
\end{proposition}


\begin{proof}
	We provide here a sketch of the proof using \citeauthor{renaud2025convergence}~\cite{renaud2025convergence}. We define the sequence shifted sequence $\boldv^{(q)})$, $q \in \mathbb{N}$ as
	\begin{equation}
		\boldv^{(q)} = \boldx^{( K_{\mathrm{ML}}  + q  )}  \, 
	\end{equation}
	and the shifted steps $\alpha_q = \delta_{   K_{\mathrm{ML}}  + q}$ which satisfies the same properties \eqref{eq:step} as $\delta^k$. Starting a modified version of Lemma~2 from \citeauthor{renaud2025convergence}~\cite{renaud2025convergence}, we have
	\begin{dmath}
		\sum_{q=0}^{N-1} \mathbb{E}  \left[ \left\| \boldv^{(q+1)} - \boldv^{(q)}     \right\|^2_2  \right]  \le 2 \alpha_0 \left(   \mathbb{E}\left[h\left(\boldv^{(0)}\right)\right] - h^\ast  \right) + \frac{4 \lambda^2 L_{\sigma}^2}{ \sigma^2}   \sum_{q=0}^{N}  \alpha_q^2 \,, 
	\end{dmath}
	where $L_{\sigma}$ is the Lipschitz constant of $D_\sigma = D_{\sigma,0}$. Using Lemma~3 from \citeauthor{renaud2025convergence}~\cite{renaud2025convergence} and $\sum_q\alpha_q^2 < +\infty$, we get 
	\begin{equation}\label{eq:bound}
		\sum_{q=0}^{N} \frac{\alpha_q}{2}\mathbb{E}  \left[ \left\|  \nabla h \left( \boldv^{(q)}  \right)    \right\|^2_2  \right] \le A  \left(\mathbb{E}\left[h\left(\boldv^{(0)}\right)\right] - h^\ast  \right) + B
	\end{equation} 
	for some $A,B\ge 0$. Combining \eqref{eq:bound} and $\sum_q\alpha_q = +\infty$ and letting $N\to+\infty$, we have $\liminf_{k\to\infty}  \left\| \nabla h \left(\boldv^{(k)} \right)  \right\|_2 = 0$ almost surely, which concludes the proof. 
\end{proof}


Now we need to prove that $\mathbb{E} \left[ \left| h\left( \boldv^{(0)} \right) \right|  \right] =  \mathbb{E} \left[\left| h\left( \boldx^{( K_{\mathrm{ML}})  } \right) \right|\right] < +\infty$. %This is a result of the smoothness assumption on $h$, in particular the Lipschitz-continuity of $D_{\sigma,\ell}$. 
We first prove  that $\mathbb{E}  \left[  \left\|\boldx^{( K_{\mathrm{ML}})} \right\|_2^2  \right] < +\infty $ by induction, starting from $\boldx^{(0)} = \boldA^\dag \boldy$ which is deterministic conditionally to the data $\boldy$. This can be achieved by observing that each iterate in Algorithm~\ref{algo:ml} and Algorithm~\ref{algo:mr} consists in a finite number of operations involving linear operators, the Lipschitz-continuous denoisers $D_{\sigma,\ell}$, the non-expensive $\operatorname{prox}_{\delta_\ell f_\ell}$ (thanks to the convexity of $f_\ell$) and independent Gaussian noise realizations with finite second-order moments. 

As $\nabla h$ is $M$-Lipshichtz for some $M$, such that  $h(\boldx) \le h(\boldzero_{\calX}) + \langle\nabla h(\boldzero_{\calX}),\boldz\rangle+\frac{M}{2}\|\boldx\|_2^2 $. Taking $\boldx =  \boldx^{(K_{\mathrm{ML}})}$ and averaging yields $\mathbb{E} \left[ h\left( \boldx^{( K_{\mathrm{ML}})} \right)\right] < +\infty$. 

A more detailed version of this proof can be found in Supplementary Material.

%The operators $\boldR_\ell$ and $\boldP_\ell$ preserve the existence of second moment. 
%
%Let $\boldx = \check{\boldx}_\ell^{(k,j)}$  for some $j$, $\ell$ and $k<K_{\mathrm{ML}}$, be the current \gls{ML} estimate   (Algorithm~\ref{algo:ml}), such that  $\mathbb{E}[\|\boldx\|_2^2]<+\infty$ as well as all previous estimates at other levels.  The Lipschiz continuity of $D_{\sigma,\ell}$ implies that $\| \boldU_{\sigma,\ell}(\boldz,\boldn_\ell) \|_2^2\le C_\ell (1 + \|\boldx\|_2^2 + \|\boldn_\ell\|_2^2) < + \infty$ for some $C_\ell>0$, which is also finite in expectation. Let $\boldu = \boldU_{\sigma,\ell}(\boldx,\boldn_\ell)$. We denote $\boldv = \boldx - \delta_{\ell} \lambda \boldu - \delta_{\ell} \boldc $ and $\boldc = \boldc_{f,\ell}^{(k)}$. % +  \lambda \hat{\boldc}_{g,\ell}^{(k)} $ with $\hat{\boldc}_{g,\ell}^{(k)} = \bar\boldR_\ell \boldU_{\sigma,0} \left( \boldx_0^{(k)} , \boldn_0 \right) - \boldU_{\sigma,\ell}  \left( \boldR_\ell \boldx_0^{(k)} , \boldn_\ell \right)$ 



%Using basic algebra and the Lipschitz continuity of $\boldU_{\sigma,0}$, %and $\boldU_{\sigma,\ell}$,
%we show that$\mathbb{E} [ \|\boldv\|_2^2 ]<+\infty$. Additional, since $f_\ell$ is convex, $\operatorname{prox}_{\delta_\ell f_\ell}$ is non-expansive, such that we can show that $\left\| \operatorname{prox}_{\delta_\ell f_\ell} ( \boldv  )  \right\|_2^2\le  2 \|\boldv\|_2^2 + 2 \left\|\operatorname{prox}_{\delta_\ell f_\ell} ( \boldzero_{\calX_{\ell}}  ) \right\|_2^2$\footnote{We used the identity $\operatorname{prox}_{f + \langle \boldc , \cdot \rangle}  (\boldz) = \operatorname{prox}_{f} (\boldz - \boldc)$} , which is finite in expectation. Thus, we demonstrated that all steps in the \gls{ML} subroutine preserves the existence of the second moments. A similar rational can be applied for the \gls{MR} initial estimate (Algorithm~\ref{algo:mr}).







==> figures/experiments/averaged_curves_cq500_30.tex <==

% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/experiments/curves/ct_40_views_metrics_curve.pdf}
%     \caption{
%     	Patient-level mean \gls{PSNR}, \gls{SSIM}, and \gls{LPIPS} versus runtime for $n_{\theta}=40$ projection views reconstruction on CQ500. Shaded bands indicate $\pm$ one patient-level \gls{SD}.
%     	}
%     \label{fig:cq500-ct40-metric-curves}
% \end{figure*}

==> figures/experiments/multilevel_schedules.tex <==
\begin{table}[H]
\centering
\footnotesize
\setlength{\tabcolsep}{6pt}
\begin{tabular}{@{}c c c c@{}}
\toprule
$n_\theta$ & $K_\ell$ & $K_{\mathrm{ML}}$ & $L$ \\
\midrule
$20,30,40$ & $5$ & \multirow{2}{*}{$6$} & \multirow{2}{*}{$3$} \\
$50$      & $3$ & & \\
\bottomrule
\end{tabular}
\caption{ML-SPnP multilevel schedules.}
\label{tab:wmlspnp_schedule}
\end{table}
